Linear Regression on Manifold Structured Data: the Impact of Extrinsic Geometry on Solutions

In this paper, we study linear regression applied to data structured on a manifold. We assume that the data manifold is smooth and is embedded in a Euclidean space, and our objective is to reveal the impact of the data manifold's extrinsic geometry on the regression. Specifically, we analyze the impact of the manifold's curvatures (or higher order nonlinearity in the parameterization when the curvatures are locally zero) on the uniqueness of the regression solution. Our findings suggest that the corresponding linear regression does not have a unique solution when the embedded submanifold is flat in some dimensions. Otherwise, the manifold's curvature (or higher order nonlinearity in the embedding) may contribute significantly, particularly in the solution associated with the normal directions of the manifold. Our findings thus reveal the role of data manifold geometry in ensuring the stability of regression models for out-of-distribution inferences.

==> sec_files/Archive.tex <==
\del{However, especially for linear dimensionality reduction methods, latent \red{? latent information?} may be lost after dimensionality reduction. \del{Consequently, there could be limitations to these approaches to out-of-distribution inferences for regression models with encoded data.}}

Main structure of this work
\begin{itemize}
    \item There is a localization principle in approximating high dimensional functions using ReLU DNNs. That is, if the approximation is ``good'' while the target function is ``non-linear'' enough, then the metric of the linear region is small.
    \item Since the localization principle, it makes since to think about local linear regression for high dimensional functions when the data lie on a low-dimensional manifold. 
    \item For the local linear regression for data on low-dimensional manifold, we show that how the curvature of the data manifold will affect the regression results.
    \item For certain cases, we prove it theoretically.
    \item Noise regularization.
\end{itemize}

Main contributions
\begin{itemize}
    \item Local principle.
    \item Theoretical understanding about how curvature affect the regression results, especially for $w_y^*$.
    \item noise regularization.
\end{itemize}


\section{Linear regression on compact manifold}
\paragraph{Motivation:} We can always interpret the neural networks except for the last linear layer $W^L \alpha(f^{L-1}) + b^L$ as linear regression steps on feature space $\widetilde{\mathcal M} := \alpha(f^{L-1}(\mathcal M))$.

Then, we may have $\alpha(f^{L-1}(\bm x)) \notin \widetilde{\mathcal M}$ if $\bm x \notin \mathcal M$. Thus, it is meaningful to analyze the $\|w_y^*\|$ in linear regression models on compact manifold.

WLOG, we assume $\mathcal M \subset \mathbb{R}^d$ is a compact manifold and we are doing the following linear regression
\begin{equation}\label{eq:original_loss}
	\argmin_{\bm w, b} \frac{1}{2N} \sum_{i=1}^N|\bm w^T \bm x_i + b - g_i|^2.
\end{equation}

\begin{proposition}\label{thm:invariant}The previous linear regression problem is invariant under unitary and shift transforms.
\end{proposition}
\begin{proof}
	Let us assume that 
	$$
	Q^T(\widetilde{\bm x_i} - b_0) =  \begin{pmatrix}
		x_i \\ y_i
	\end{pmatrix},
	$$
	where $Q = (Q_x, Q_y) \in \mathbb{R}^{d\times d}$ is a unitary matrix, $b_0 \in \mathbb{R}^d$, $x \in \mathbb{R}^{d_x}$,  and $y \in \mathbb{R}^{d_y}$.
	By denoting $\bm x = \begin{pmatrix}
		x_i \\ y_i
	\end{pmatrix} $, we have 
	\begin{equation*}
		\begin{aligned}
			&\min_{\widetilde{\bm w}, \tilde b} \frac{1}{2N} \sum_{i=1}^N|\widetilde{\bm w}^T \widetilde{\bm x_i} + \widetilde{b} - g_i|^2 \\
			=&\min_{\widetilde{\bm w}, \tilde b} \frac{1}{2N} \sum_{i=1}^N|\widetilde{\bm w}^T (b_0+Q\bm x_i) + \widetilde{b} - g_i|^2 \\
			=&\min_{\widetilde{\bm w}, \tilde b} \frac{1}{2N} \sum_{i=1}^N|\widetilde{\bm w}^TQ \bm x_i + \widetilde{\bm w}^Tb_0 + \widetilde{b} - g_i|^2 \\
			=&\min_{{\bm w}, b} \frac{1}{2N} \sum_{i=1}^N|{\bm w}^T \bm x_i + {b} - g_i|^2.
		\end{aligned}
	\end{equation*}
The last identity holds because of the following bijection between $\{\bm w, b\}$ and $\{\widetilde{\bm w}, \tilde b\}$ that
$$
\bm w = \widetilde{\bm w}^TQ,  \quad b = \widetilde{\bm w}^Tb_0 + \tilde b.
$$
\end{proof}

\paragraph{Basic idea:} If the curvature for the  compact manifold is small, then the manifold can be approximated by a linear space $Q_x$ with variants in the normal direction $Q_y = Q_x^\perp$. Thus, the data can be understood as 
\begin{equation}\label{key}
	\bm x = \begin{pmatrix}
		x \\ y
	\end{pmatrix}, \quad \text{with} \quad \|y\| \le \sigma_k.
\end{equation}
where $x \in \mathbb{R}^{d_x}$ and $y \in \mathbb{R}^{d_y}$. Here, we can imagine that $\sigma$ could be bounded by the curvature or just reach information. 

\begin{notation}\label{notation:1}
Let $z$ be a random variable in $\mathbb{R}^m$ or $\mathbb R^{m\times n}$ over some probability space and let $z_i$ denote a sample realization of $z$. We denote the empirical average
\begin{equation*}
    \left < z\right >_N := \frac{1}{N}\sum_{i=1}^N z_i
\end{equation*}
and the mean
\begin{equation*}
    \left <z \right > :=\lim_{N\rightarrow\infty} \left < z\right >_N = \mathbb{E}[z].
\end{equation*}
\end{notation}
\begin{notation}\label{notation:2}
For vectors $(x_i,y_i)\in \mathbb{R}^{d_x} \times \mathbb R^{d_y}$, $i=1,2,\cdots, N,$ we denote the averaged correlation matrix by
\begin{equation*}
	\left <A(x,y)\right >_N := \begin{pmatrix}
	\left <xx^T\right >_N & \left <xy^T\right >_N \\
	\left <yx^T\right >_N & \left <yy^T\right >_N
	\end{pmatrix}.
\end{equation*}
Unless explicitly stated otherwise, we will refer to $\left <A(x,y)\right >_N$ as $\left <A\right >_N$.
\end{notation}

\subsection{Warm up}
For example, let us denote 
\begin{equation}\label{key}
	\mathcal M  = \{(\frac{1}{\kappa}\cos(\theta),  \frac{1}{\kappa}\sin(\theta)) ~:~  \theta_0 - \delta \le \theta \le \theta_0 + \delta\},
\end{equation}
where $\kappa = \frac{1}{r}$ is the curvature of the circle with radius $r$. Then, we have 
\begin{equation}\label{key}
	|y| \le (1-\cos(\delta)) \frac{1}{2\kappa}.
\end{equation}
Notice that 
\begin{equation}\label{key}
	2 \delta \frac{1}{\kappa} = \left|\mathcal M\right|
\end{equation}
and $\delta < < 1$. Finally, we have
\begin{equation}\label{key}
	|y| \lesssim \left|\mathcal M\right|^2 \kappa
\end{equation}

Or, I am thinking to introduce the reach $r$ to control $\|y\|$ locally which is similar to the theorem that Lewis introduced two weeks ago...

\paragraph{Another argument about why $|y| \sim \mathcal O(\kappa)$.} 
Here, we can consider the Taylor expansion of  $\bm x = (r\cos(\theta), r\sin(\theta))$ at $\theta = \theta_0$ as
\begin{equation}\label{eq:expansion_x}
	\begin{aligned}
	\bm x &= \begin{pmatrix}
		r\cos(\theta) \\ r\sin(\theta)
	\end{pmatrix} \\
 &= \begin{pmatrix}
	r\cos(\theta_0) \\ r\sin(\theta_0)
	\end{pmatrix} + \begin{pmatrix}
	-\sin(\theta_0) \\ \cos(\theta_0)
\end{pmatrix}r(\theta-\theta_0) 
	+ \begin{pmatrix}
		-\cos(\theta_0) \\ -\sin(\theta_0)
	\end{pmatrix}r(\theta-\theta_0)^2 + \cdots
	\end{aligned}
\end{equation}
Here, we denote $Q_x = \begin{pmatrix}
	-\sin(\theta_0) \\ \cos(\theta_0)
\end{pmatrix}$ and $Q_y = \begin{pmatrix}
-\cos(\theta_0) \\ -\sin(\theta_0)
\end{pmatrix}$. Correspondingly, we have $x = r(\theta-\theta_0)$ and $y = r(\theta-\theta_0)^2$. 
\begin{assumption}[Informal]
	Let us assume that $x \sim \mathcal O(1)$. 
\end{assumption}
Under this assumption, we have $(\theta-\theta_0) \sim \mathcal O\left(\frac{1}{r}\right)  = \mathcal O\left(\kappa\right)$ which leads to 
\begin{equation}\label{key}
	y = r(\theta-\theta_0)^2 \sim (\theta-\theta_0) \sim \mathcal O\left(\kappa\right).
\end{equation}

\paragraph{Main differences from the linear case:} $y = y(x)$ under the previous decomposition. Thus, it is hard to introduce $y$ just as a pure noise. As a result, we can only have
\begin{equation}\label{key}
	\left <xy^T\right >_N \le \sigma_k
\end{equation}
while $\left <xy^T\right >_N \le \frac{\sigma_n}{\sqrt{N}}$ in linear case since $y\sim N(0,\sigma_n^2)$ is the artificial noise.
Here, we denote $\sigma_k$ as the derivation of $y$ component introduced by the curvature while $\sigma_n$ is the standard derivation of the artificial noise.

For this case, we have $ \bm w^* = \left <A\right >_N^{-1} \left <(g-b)\bm x\right >_N$ where 
\begin{equation}\label{key}
	\left <A \right >_N = \begin{pmatrix}
		\left <xx^T\right >_N & \left <xy^T\right >_N \\
		\left <yx^T\right >_N & \left <yy^T\right >_N
	\end{pmatrix}, \quad b = \left <g\right >_N - \bm w^T \left <\bm x\right >_N.
\end{equation}
If $\bm x$ is the real data, then we can make the assumption that $\left <\bm x\right >_N$ since we can apply the normalization preconditioning for the data set. However, if $\bm x = \alpha{f^{L-1}(\bar x)}$ is in the feature space, then we have 
$$
\left <\bm x\right >_N = \left<\alpha{f^{L-1}(\bar x)}\right >_N  > 0, 
$$
since $\alpha(t) = {\rm ReLU}(t)\ge 0$. For this case, we have 
$$
\bm w^* = (\left <A\right >_N - \left <\bm x\right >_N\left <\bm x\right >_N^T)^{-1}\left <\left(g-\left <g\right >_N\right)\bm x\right >_N
$$
Then, we may need the S-M-W formula...
\blue{more details to be added...}

Here, we may prove that 
$$
\|w_y^*\| \lesssim \frac{1}{\sigma_k} \approx \mathcal O \left(\frac{1}{\kappa}\right).
$$
This is consistent with the linear case, since $\kappa = 0$ then $\|w_y^*\|$ losses the control in pure linear regression case.

\subsection{Another approach} Let us assume that the feature manifold can be parameterized as 
$$
\bm x = \begin{pmatrix}
	x \\ y=h(x)
\end{pmatrix}
$$
after a shift and unitary transform. Furthermore, we may choose a proper shift and unitary transform such that
$$
 \left <x\right > = 0, \quad h(0) = 0 \in \mathbb{R}^{d_y}, \quad \nabla h(0) = 0 \in \mathbb{R}^{d_y\times d_x}.
$$
Thus, the Taylor expansion of $y = h(x)$ can be written as
$$
y = h(x) = h(0) +  \nabla h(0) x + x \cdot \nabla^2 h(0) \cdot x + \cdots.
$$
The key observation is that $x\sim \mathcal O(1)$ and $ \nabla^2 h(0)$ is determined (bounded) by the curvature tensor $\kappa$.
Here, we recall the previous example that $\bm x = (r\cos(\theta), r\sin(\theta))$. In that example, we have $x = r(\theta-\theta_0)$ and 
$$
y = r(\theta-\theta_0)^2 = \frac{1}{r}x^2 = \kappa x^2 = x \cdot \nabla^2 h(0) \cdot x.
$$


\lewis{The below materials are my new editions.}

==> sec_files/invariant_W1.tex <==
\section{Special manifold and invariance in $W^1$}
First, let us recall the ReLU DNN function with $L-1$ hidden layers as  
\begin{equation}\label{eq:DNN}
	\begin{cases}
		f^{\ell}(\bm x) &= W^\ell \alpha(f^{\ell-1}(\bm x) ) + b^{\ell}, \quad \ell = 2:L, \\
		f (\bm x,\theta) &= f^{L}(\bm x),
	\end{cases}
\end{equation}
where $f^1(\bm x) = W^1\bm x + b^1$, $\alpha = {\rm ReLU}$, $W^\ell \in \mathbb R^{n_{\ell}\times n_{\ell-1}}$, $b^\ell, f^\ell \in\mathbb{R}^{n_{\ell}}$ with $n_0=d=d_x+d_y$ and $n_L=1$.

Then, the loss function is defined as
\begin{equation}\label{eq:lossf}
	J(\theta) =\frac{1}{2N} \sum_{i=1}^{N} ( f(\bm x_i; \theta) -g_i )^2 = \frac{1}{2N} \sum_{i=1}^{N} J_i(\theta),
\end{equation}
where $\theta = \{W^1, b^1, \cdots, W^L, b^L\}$ denotes all parameters in ReLU DNNs and 
$$
J_i(\theta) = ( f(\bm x_i; \theta) -g_i )^2.
$$

Let us denote the following manifold:
\begin{equation}\label{eq:M}
	\mathcal M = \left\{ \bm x ~:~ \bm x^T F_k(\bm x) = 0, \quad k=1:d_y\right\},
\end{equation}
where 
$$
F_k: \mathbb R^d \mapsto \mathbb{R}^d, \quad \text{ is smooth}.
$$
\begin{itemize}
	\item If $F_k(\bm x) = a_k$ as a constant vector function, then  $\mathcal M$ degenerates to a linear subspace. 
	\item We also notice that for any algebraic varieties that contain the origin $\bm 0$ can be written as this form.
\end{itemize}

\paragraph{Key observation:} If $\bm x_i \in \mathcal M$, then 
\begin{equation}\label{key}
	\frac{\partial J_i(\theta)}{\partial \left(W_j^1\cdot F_k(\bm x_i)\right)} = 0, \quad \forall k=1:d_y, j=1:n.
\end{equation}

However, this is only a local property for the invariant of $W^1$ since $F_k(\bm x_i)$ are different for different data point $\bm x_i$.



==> sec_files/localization.tex <==
\section{Localization principle in ReLU DNNs}
\Lewis{section as motivations}
\Lewis{\begin{itemize}
    \item observed concentration around low-d manifold, common assumption in manifold learning community
    \item still common to study linear regression
    \item linear regression related to ReLU DNN
    \item reference from manifold learning: wenjing liao; alex krodinger; reach too strong/global; moving least square(?)
    \item Investigate two questions: when the problem is well-posed; how does noise affect well/ill-posedness
    \item extrinsic geometry matters more when noises presence
    \item build up theories for different cases
\end{itemize} }
First, we assume that the date distribution satisfies
\begin{equation}
    \label{eq:D}
    c\delta \le \min_{j\neq i} \|x_i - x_j\| \le C\delta
\end{equation}
for any data points $x_i \in \Omega$ with $i=1:N$. Here, we notice that $\delta \to 0$ if $N\to \infty$ since $\Omega$ is a compact set.
In addition, we also assume that the trained error of the ReLU DNN function $f(x)$ on data set $D:= \{(x_i, g(x_i))\}_{i=1}^N$ has
\begin{equation}\label{eq:J}
J = \frac{1}{N}\sum_{i=1}^N (f(x_i) - g(x_i))^2 \le \epsilon^2.
\end{equation}
Furthermore, we denote
\begin{equation}\label{eq:J_i}
J_i = |(f(x_i) - g(x_i)| \le \epsilon_i,
\end{equation}
and $\epsilon_i \le A \epsilon$ for some constant $A > 0$.

Denote $K_{i}$ as the largest simply connected domain such that 
\begin{equation}
    \nabla f(x_i) = \nabla f(x), \quad x \in K_{i}.
\end{equation}
Denote $|K_i|$ as the $n$-dimensional volume of $K_i$. Then, we have $|K_i| = 0$ if $\nabla f(x_i) $ does not exists, i.e., $x_i$ lies on the boundary of the mesh produced by the piecewise linear function $f(x)$. If $|K_i|>0$, we hope to find an upper bound for $|K_i|$.

The key observation is
\begin{equation}
    \inf_{f(x)=w^Tx+b}\|f(x) - g(x)\|_{L^2(K)} \approx h^2 |g|_{2,K},
\end{equation}
where $h := \max_{x,y\in K}\|x-y\|$ and $K$ is a simplex in $\mathbb R^d$. That is, if $|g|_{2,K}$ is large then it is necessary to have a small local linear approximation for a small error.
Typically, the upper bound $h^2|g|_{2,K}$ is easy to obtained. However, it is actually also bounded below. \blue{I will check more details about this result in finite element.}


\begin{theorem}[informal]
Assume that $f(x)$ is the trained ReLU DNN that satisfies \eqref{eq:J} and \eqref{eq:J_i}. Furthermore, if $\epsilon = 0$ and $N$ is large and the ReLU DNN $f(x)$ is sufficient large (over-parameterization), then the diameter of $K_i$ denoted as 
$$
d_i := \max_{x, y\in K_i}\|x-y\| \lesssim \frac{1}{\sqrt{N|g|_{2,K_i}}}.
$$
\end{theorem}
\begin{proof}According to the bound of generalization of ReLU DNN (for example Barron 93), we have $$
\|f - g\|_{L^2(\Omega)} \lesssim \frac{1}{\sqrt{N}} + \text{approximation error}.
$$
Since we assume $f(x)$ is a relatively large model (over-parameterization), we see that $\frac{1}{N}$ dominates the error. Thus, we have
$$
\frac{1}{\sqrt{N}} \ge \|f - g\|_{L^2(\Omega)} \ge \|f-g\|_{L^2(K_i)} \ge d_i^2|g|_{2,K_i},
$$
as $f(x)$ is a linear function on $K_i$.
Therefore, we have
$$
d_i \lesssim \frac{1}{\sqrt{N|g|_{2,K_i}}}.
$$
\end{proof}

% Some further questions:
% \begin{itemize}
%     \item How about $\epsilon > 0$?
%     \item Can we involve features of discrete data set, for example, $\delta$ as in \eqref{eq:D}?
% \end{itemize}


% \subsection{How the information of derivatives affects the mesh in ReLU DNN}
% Since a ReLU DNN function is a piecewise linear function, we can regard the trained ReLU DNN function as the result of adaptive linear finite element method (AFEM). In AFEM, we first introduce the equidistribution principle. Given function $u \in W^{2,1}(\Omega)$ and a triangular mesh $\mathcal T_N$ with $N$ elements on $\Omega \subset \mathbb R^2$, let $u_I$ be the linear nodal value interpolation of $u$ on $\mathcal T_N$. For any triangle $K \in \mathcal T_N$, we have
% \begin{equation}
%     |u - u_I|_{1,K} \lesssim |u|_{2,1,K}
% \end{equation}
% if $K$ is shape-regular. Thus, we have
% $$
% |u-u_I|_{1,\Omega}^2 \lesssim \sum_{K\in \mathcal T_N} |u|^2_{2,1,K}.
% $$


